A Data-Based Perspective on Transfer Learning

It is commonly believed that in transfer learning including more pre-training data translates into better performance. However, recent evidence suggests that removing data from the source dataset can actually help too. In this work, we take a closer look at the role of the source dataset's composition in transfer learning and present a framework for probing its impact on downstream performance. Our framework gives rise to new capabilities such as pinpointing transfer learning brittleness as well as detecting pathologies such as data-leakage and the presence of misleading examples in the source dataset. In particular, we demonstrate that removing detrimental datapoints identified by our framework improves transfer learning performance from ImageNet on a variety of target tasks. Code is available at https://github.com/MadryLab/data-transfer

==> sections/5_19_framework.tex <==
In order to pinpoint how the source dataset's composition impacts transfer learning, we need to untangle the relationship between the source datapoints and the transfer model's performance. 
To do so, we draw inspiration from a line of work which, in non-transfer settings, seeks to quantify how including or excluding a certain training datapoint changes a model's test prediction. This line of work includes approaches such as influence functions~\cite{cook1982residuals, koh2017understanding, feldman2020what}, datamodels~\cite{ilyas2022datamodels}, and the computation of data-Shapley values~\cite{kwon2021beta, karlavs2022data, ghorbani2019data}.

We now want to adapt this paradigm to analyze transfer learning. To do so, we seek to capture how including or excluding source datapoints impacts performance on the target task. Note that, in the transfer learning setting, the contribution of the source model is not individual predictions, but instead learned features that are later leveraged for the downstream task. These features are unlikely to change with the removal of individual source datapoints. Thus, we would like to instead remove collections of datapoints that together contribute to meaningful features. 
We therefore focus on entire source classes. Specifically, we seek to estimate an influence value for each \emph{source class} that captures how its presence changes the transfer model's prediction on each \emph{target example}.

So how can we compute the influence of a source class? A natural way to do this is to remove a single class and then measure the change in transfer performance. However, this approach can fail if there are very similar classes in the dataset---as is the case in ImageNet---because the downstream task will still be able to leverage the shared feature learned the from the other classes. To avoid this issue, we instead remove many classes at the same time.

\paragraph{Computing transfer influences.} Motivated by this, we train a large number\footnote{7540 models in this paper. Details and convergence analysis are in Appendix~\ref{app:setup}.} of models with random subsets of the source classes, and then fine-tune these models to get their predictions on the target task. With these predictions, we are now ready to compute the influence of a source class on transfer learning. Specifically, we estimate the influence value of a source class $\mathcal{C}$ on a target example $t$ as the expected difference in the transfer model's performance on $t$ when $\mathcal{C}$ was either included or excluded from the source dataset:
\begin{align}
    \label{eq:influence}
    \text{Infl}[\mathcal{C} \rightarrow t] = \mathbb{E}_{S} \left[ f(t; S) ~|~ \mathcal{C} \subset S \right] - \mathbb{E}_{S} \left[ f(t; S) ~|~ \mathcal{C} \not \subset S \right]
\end{align}
where $f(t; S)$ is the softmax\footnote{We experiment with other outputs such as logits, margins, or correctness. We defer the details to Appendix~\ref{app:variants-influences}.} output of a model trained on a random subset $S$ of the source dataset. A positive influence value indicates that including the source class helps the model predict the target example correctly. In contrast, a negative influence value suggests that the source class actually hurts the model's performance on the target example.  We outline the overall procedure in Algorithm~\ref{alg:main}, and defer a detailed description of our approach to Appendix TODO.



% Once we have calculated these influence values, we can now leverage them to both understand and improve transfer learning. In the following sections, we demonstrate that influences can be used to boost transfer performance by removing detrimental data, identify subpopulations in the target dataset that were particularly impacted by a source class, debug transfer mistakes, and even identify data leakage between the source and target datasets. 




\begin{algorithm}[!hbtp]
    \caption{Influence estimation of source dataset classes on transfer learning.}
    \label{alg:main}
    \begin{algorithmic}[1]
    \Require source dataset $\mathcal{S} = \cup_{k=1}^{K}~\mathcal{C}_k$ (with $K$ classes), a target dataset $\mathcal{T} = (t_1, t_2,\cdots,t_n$), training algorithm $\mathcal{A}$, subset ratio $\alpha$, number of models $m$
    \State Sample $m$ random subsets of $S_1,S_2,\cdots,S_m \subset \mathcal{S}$ of size $\alpha \cdot |\mathcal{S}|$: 
    \For{$i \in  1$ to $m$}
        \State Train model $f_i$ by running algorithm $\mathcal{A}$ on $S_{i}$
    \EndFor
    \For{$k \in  1$ to $K$}
    \For{$j \in  1$ to $n$}
        \State$ \text{Infl}[\mathcal{C}_k \rightarrow t_j] =
        \frac{
            \sum_{i=1}^{m} f_i(t_j; S_i) \mathbbm{1}_{\mathcal{C}_k \subset S_i}
        }{\sum_{i=1}^m \mathbbm{1}_{\mathcal{C}_k \subset S_i}
        } - \frac{
            \sum_{i=1}^{m} f_i(t_j; S_i) \mathbbm{1}_{\mathcal{C}_k \not \subset S_i}
        }{\sum_{i=1}^m \mathbbm{1}_{\mathcal{C}_k \not \subset S_i}} $
    \EndFor
    \EndFor
    \State
    \Return $\text{Infl}[\mathcal{C}_k \rightarrow t_j]~~\forall~~j\in[n], k\in[K]$
    \end{algorithmic}
\end{algorithm}


==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/old_framework.tex <==
Conventional wisdom suggests that larger source datasets result in better downstream transfer performance~\cite{sun2017revisiting,mahajan2018exploring}.  But, recent works \citep{huh2016makes, ngiam2018domain,kolesnikov2019big} have shown that this is not always the case. For example, \citet{ngiam2018domain} find that hand-picking subsets of the source dataset can boost transfer performance over using the original source dataset in its entirety. Thus, the composition of the source dataset (and not just its size) plays an important role in transfer learning. So, which source datapoints should we choose for a  particular target task?

In this paper, we analyze how datapoints in the source dataset can positively (or negatively) impact performance on the target task. Specifically, we estimate the \textit{influence} of source datapoints (or groups of datapoints, e.g., classes) on downstream predictions by studying how the inclusion of those datapoints changes the model's behavior on downstream target tasks. In Section~\ref{sec:counterfactuals}, we show that removing ``negative influencers,'' i.e., datapoints that negatively affect downstream predictions, from the source dataset can improve transfer performance. Then in Section~\ref{sec:science}, we demonstrate how we can use our framework to derive insights about what drives transfer learning.

% \sam{A bit of a conceptual jump after here. So far it is only about choosing datapoints (so a reader might naturally think of choosing indiv points), but from here on it's all about classes. So say something about: we're gonna look at groups/subpopulations of examples, and here we're gonna focus on a natural grouping, classes--or something to that effect. I do see the footnote but I think it might be better to be more explicit.}
\paragraph{Measuring the influence of the source dataset.}
Given a source dataset $\mathcal{S}$ consisting of $K$ classes $\mathcal{C}_1, ..., \mathcal{C}_K$ and a target dataset $\mathcal{T}$, the key idea of our framework is to define and estimate \textit{influence values} $\text{Infl}[\mathcal{C}_k \rightarrow t]$, which capture the impact that each class $\mathcal{C}_K$ in the source dataset has on the predictions of each target datapoint $t \in \mathcal{T}$.\footnote{While here we consider the influence of source \textit{classes}, we can adapt our framework to instead estimate the impact of specific source \textit{examples} on the target predictions. See Section~\ref{sec:example_wise}.}

One natural way to estimate such influence values is to measure the change in transfer performance when we remove a single class from the source dataset. However, this ``leave-one-out'' approach would not successfully isolate the contribution of classes that contain redundant information with other classes. For example, removing only one of the ImageNet classes that is a sub-breed of dog (e.g., ``poodle'' or ``golden retriever'') may have a negligible effect on the transfer model's predictions to a target dataset containing dogs. However, removing all of the dog ImageNet classes together might significantly change the transfer model's behavior.
% However, as we show in Appendix~TODO, removing a single class at a time has a relatively marginal impact on the overall transfer performance. For 1000 classes, running enough models to see meaningful signal for this leave-one-out approach would be prohibitively expensive. Moreover, we would like to capture the impact of classes in conjunction with other classes in the source dataset. For example, the class ``golden retriever'' might have a trivial effect when removed alone, but might significantly change the transfer model's behavior when removed alongside other dog breed classes.

We would therefore like to capture the impact of classes in conjunction with other classes in the source dataset, thus amplifying the effect of removing a specific class. So, instead of removing one class at a time, we remove collections of classes at once by training on \textit{subsets} of the source dataset. Specifically, we train many models\footnote{Roughly 7800 models in this paper. Details and convergence analysis are in Appendix~\ref{app:setup}.} on random subsets of the source dataset---where each subset only contains a fixed number of classes---and then finetune each of these models on the target task. Each class $\mathcal{C}_k$ is included in the source dataset of some of these transfer models, but not in the rest. Finally, we record each transfer model's predictions on the target dataset. Using this information, we estimate the influence $\text{Infl}[\mathcal{C}_k \rightarrow t]$ of class $C_k$ on a target example $t \in \mathcal{T}$ as the expected difference in the performance on $t$ when $C_k$ is included or excluded from the source dataset:
\begin{align}
    \label{eq:influence}
    \text{Infl}[\mathcal{C}_k \rightarrow t] = \mathbb{E}_{\mathcal{S}_i} \left[ f(t; \mathcal{S}_i) ~|~ \mathcal{C}_k \subset \mathcal{S}_i \right] - \mathbb{E}_{\mathcal{S}_i} \left[ f(t; \mathcal{S}_i) ~|~ \mathcal{C}_k \not \subset \mathcal{S}_i \right]
\end{align}
where $f(t; \mathcal{S}_i)$ is the softmax\footnote{We experiment with other outputs such as logits, margins, or correctness. We defer the details to Appendix~\ref{app:variants-influences}.} output of a model trained on a subset $\mathcal{S}_i$ of the source dataset $\mathcal{S}$. We outline the overall procedure in Algorithm~\ref{alg:main}.

% {\color{blue}SP: I wrote the following two sentences to make more paralellel and concise. Old version is commented out.}
A positive $\text{Infl}[C_k\rightarrow t]$ indicates that including $C_k$ in the source dataset improves models' performance on target example $t$ on average. In contrast, a negative $\text{Infl}[C_k\rightarrow t]$ indicates that including $C_k$ hurts models' performance on example $t$.
%If $\text{Infl}[C_k\rightarrow t]$ is positive, then models that included $C_k$ in the source dataset performed on average better on the target example $t$ than those that did not include $C_k$. In contrast, negative values of $\text{Infl}[C_k\rightarrow t]$ indicate that including $C_k$ hurts the model's performance on the example $t$.
We further denote $\text{Infl}[C_k]$ as the average of the influences $\text{Infl}[C_k\rightarrow t]$ over all examples $t\in\mathcal{T}$ in the target dataset. This allows us to capture the effect of $\mathcal{C}_k$ on the overall downstream transfer performance.

% By computing an influence estimate for every class of the source dataset on each datapoint in the target dataset, we can uncover which classes are most/least important for the  model's transfer performance. We will later see how this allows us to improve transfer learning by removing the least important classes from the source dataset. We will also demonstrate other uses for these class influences estimates.

Our framework is inspired by influence functions~\cite{koh2017understanding,feldman2020what} and datamodels~\cite{ilyas2022datamodels}. These works estimate the influence of specific training datapoints on model predictions in standard ML (non-transfer) settings. In contrast to these works, we instead consider the transfer learning setting and leverage influences to study the impact of the source dataset composition on the model's downstream predictions.


\begin{algorithm}[t]
    \caption{Influence estimation of source dataset classes on transfer learning.}
    \label{alg:main}
    \begin{algorithmic}[1]
    \Require source dataset $S = \cup_{k=1}^{K}~\mathcal{C}_k$ (with $K$ classes), a target dataset $\mathcal{T} = (t_1, t_2,\cdots,t_n$), training algorithm $\mathcal{A}$, subset ratio $\alpha$, number of models $m$
    \State Sample $m$ random subsets of $S$ of size $\alpha \cdot |\mathcal{S}|$: $S_1,S_2,\cdots,S_m$
    \For{$i \in  1$ to $m$}
        \State Train model $f_i$ by running algorithm $\mathcal{A}$ on $S_{i}$
    \EndFor
    \For{$k \in  1$ to $K$}
    \For{$j \in  1$ to $n$}
        \State$ \text{Infl}[\mathcal{C}_k \rightarrow t_j] =
        \frac{
            \sum_{i=1}^{m} f_i(t_j; \mathcal{S}_i) \mathbbm{1}_{\mathcal{C}_k \subset \mathcal{S}_i}
        }{\sum_{i=1}^m \mathbbm{1}_{\mathcal{C}_k \subset \mathcal{S}_i}
        } - \frac{
            \sum_{i=1}^{m} f_i(t_j; \mathcal{S}_i) \mathbbm{1}_{\mathcal{C}_k \not \subset \mathcal{S}_i}
        }{\sum_{i=1}^m \mathbbm{1}_{\mathcal{C}_k \not \subset \mathcal{S}_i}} $
    \EndFor
    \EndFor
    \State
    \Return $\text{Infl}[\mathcal{C}_k \rightarrow t_j]~~\forall~~j\in[n], k\in[K]$
    \end{algorithmic}
\end{algorithm}

==> sections/quantifying.tex <==
In Section~\ref{sec:framework}, we presented a framework for pinpointing the role of the source dataset in transfer learning by estimating the influence of each source class on the model's target predictions. In this section, we demonstrate how our framework can enable us to identify the classes in the source dataset that, positively or negatively, have a largest impact on the overall transfer performance. 

In particular, recall that the influence value that we estimated in Section \ref{sec:framework} reflects whether the inclusion of the source class, on average, improved or hurt the transfer model's performance on a particular target example. If we average these influences across the entire target dataset, we can identify the \textit{overall} most influential source classes for transfer learning.


\begin{figure}[!t]
    \begin{minipage}[t]{0.8\textwidth}
        \vspace{0pt}
        \includegraphics[width=\linewidth]{figures/qualitative/paper_barplots/overall.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.19\textwidth}
        \vspace{0pt}
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{cc}
            \multicolumn{2}{c}{CIFAR-10 Classes}\\
            \hline
            airplane & dog \\ 
            automobile & frog \\  
            bird & horse \\   
            cat & ship  \\
            deer & truck  \\  
        \end{tabular}
    \end{minipage}
    \caption{We display the top and bottom classes of ImageNet ordered based on their overall influence values on the CIFAR-10 dataset. The top ImageNet classes are semantically relevant to the CIFAR-10 classes. A similar plot for each CIFAR-10 class separately can be found in Figure~\ref{fig:class-barplots} and Appendix~\ref{app:omitted}.}
    \label{fig:influencers-cifar-overall}
\end{figure}

We find that not all source classes are equally important for transfer learning. In Figure \ref{fig:influencers-cifar-overall}, we display the most positively and negatively influential classes for ImageNet when performing transfer to CIFAR-10.  In particular, we note that the most positively influential classes are directly relevant to classes in the CIFAR-10 task (i.e., the ImageNet label \textit{tailed frog} is an instance of CIFAR class \textit{frog}). We find that this trend holds across target datasets (see Appendix~\ref{app:counterfactual_all_datasets} for more datasets and for full-feature transfer results). 

We can also identify source classes which are overall negative influencers for the target dataset (e.g., \textit{bookshop} and \textit{jigsaw puzzle}). These classes are often negative influencers over many types of images in the target dataset. For example, \textit{bookshop} is in the top 10 most negative influencers for 7 out of the 10 CIFAR-10 classes (see Appendix TODO). In Section~\ref{sec:science}, we take a closer look at the factors that can cause a source class can be a negative influencer for a target prediction.

\paragraph{Validating transfer influences through counterfactual experiments.} How well do these influence values actually reflect the importance to the overall transfer performance? To answer this question, we remove ImageNet classes from the source dataset in the order of highest or lowest influence/ We display these results with CIFAR10 as the target-task in Figure~\ref{fig:cifar_detailed_fixed_cf}. We find that removing the top influential classes severely degrades transfer performance over removing random classes, which confirms their importance to the transfer learning process. In contrast, removing the bottom classes allows us to improve the overall transfer performance \emph{even beyond using the entire ImageNet dataset}.  In Figure~\ref{fig:summary_fixed_cf}, we find that across target tasks, we can improve transfer performance by removing the most negatively influential classes. \saachi{should we mention the hand-picked baseline here?}


% \paragraph{A hand-picked baseline.} Above, we noted that the top influential classes of the source dataset are typically relevant to the classes in the target dataset. What happens if we choose our source dataset by \textit{hand-picking} ImageNet classes that are relevant to the target dataset? Indeed, \cite{ngiam2018domain} found that hand-picking such source datasets can sometimes boost transfer performance. To check this for our setting, we choose the ImageNet classes that are children of the target classes in the WordNet hierarchy\cite{miller1995wordnet} (see Appendix~\ref{app:setup} for details). We display this hand-picked baseline for CIFAR-10 in Figure~\ref{fig:cifar_detailed_fixed_cf}, and the other datasets in Appendix~\ref{app:counterfactual_all_datasets}. We find that choosing an optimal subset of classes via influences substantially outperforms the hand-picked baseline.



\begin{figure}[!t]
    \begin{subfigure}[c]{0.48\linewidth}
        \vspace{0pt}
        \includegraphics[width=\linewidth]{figures/quantitative/CIFAR10_transfer_results_cf.pdf}\hfill
        \caption{CIFAR-10 results}
        \label{fig:cifar_detailed_fixed_cf}
    \end{subfigure}\hfill
    \begin{subfigure}[c]{0.48\linewidth}
        \vspace{0pt}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|cc}
            \toprule
            & \multicolumn{2}{c}{\textit{Source Dataset}}\\
            \textit{Target Dataset} & Full ImageNet & \makecell{Removing \\Bottom Infl.}\\
            \midrule
            AIRCRAFT & $36.08 \pm 0.66$ & $\mathbf{36.88 \pm 0.46}$ \\
            BIRDSNAP & $38.42 \pm 0.24$ & $\mathbf{39.19 \pm 0.24}$ \\
            CALTECH-101 & $86.69 \pm 0.49$ & $\mathbf{87.03 \pm 0.18}$ \\
            CALTECH-256& $74.97 \pm 0.17$ & $\mathbf{75.24 \pm 0.13}$ \\
            CARS & $39.55 \pm 0.20$ & $\mathbf{40.59 \pm 0.32}$ \\
            CIFAR-10 & $81.16 \pm 0.19$ & $\mathbf{83.64 \pm 0.22}$ \\
            CIFAR-100 & $59.37 \pm 0.36$ & $\mathbf{61.46 \pm 0.35}$ \\
            FLOWERS & $\mathbf{82.92 \pm 0.32}$ & $82.89 \pm 0.29$ \\
            FOOD & $56.19 \pm 0.09$ & $\mathbf{56.85 \pm 0.16}$ \\
            PETS & $83.41 \pm 0.34$ & $\mathbf{87.59 \pm 0.15}$ \\
            SUN397 & $50.15 \pm 0.14$ & $\mathbf{51.34 \pm 0.18}$ \\
            \bottomrule
        \end{tabular}
        }
        \caption{Summary of 11 target tasks}
        \label{fig:summary_fixed_cf}
    \end{subfigure}

    \caption{We compute influence values for ImageNet classes on various target tasks. We remove ImageNet classes in order of top (most positive) or bottom (most negative) overall influence values, and then fine-tune using this subset as the source dataset for transfer learning. We compare against using the full ImageNet dataset, a random subset, or a hand-picked subset of relevant classes based on the WordNet hierarchy (see Appendix TODO for details). Results are reported over 10 runs, with 95\% confidence intervals. \textbf{(a)} Results with CIFAR-10 as the target task, removing various numbers of classes from the source dataset. Max improvement is the peak improvement of removing the bottom influencers vs. using the full ImageNet dataset. Results for other target tasks can be found in Appendix~\ref{app:counterfactual_all_datasets}. \textbf{(b)} Summary of the peak performance from removing the bottom influencers across a range of target tasks.}
    \label{fig:cf_fixed_cifar}
\end{figure}

\paragraph{Generalization of ImageNet class influences.} How task-specific are the most influential source classes? In Appendix TODO, we repeat the counterfactual experiments in Figure~\ref{fig:cf_fixed_cifar}, but instead of computing influences for each task separately, we use the influences computed for ImageNet $\rightarrow$ CIFAR-10 for the other downstream tasks. While we find that these proxy influences are more informative than a random baseline, we achieve the best results for when using the actual task for influence computation. Thus, these influences do contain task-specific information. We examine other generalization across architectures and across transfer types in Appendix~\ref{app:influence-transfer}.


\

% \begin{figure}[!t]
%     \includegraphics[width=\textwidth]{figures/qualitative/barplots/class_0.pdf}
%     \includegraphics[width=\textwidth]{figures/qualitative/barplots/class_2.pdf}
%     \caption{Top and bottom influencers for two CIFAR-10 classes from the ImageNet classes that are related to the CIFAR-10 class (e.g., ``airliner''/``warplane'' for the CIFAR-10 class ``airplane''). The negative influences on the other hand are unrelated classes. This fits the intuition that for a closer source dataset to the target task, the better the transfer performance.
%     }
%     \label{fig:influencers-cifar-perclass}
% \end{figure}
